Connectivity estimation of high dimensional data recorded from neuronal cells

The main result of this thesis is the development of a novel connectivity estimation method, called Total Spiking Probability Edges (TSPE). Based on cross-correlation and edge filtering at different time scales this method is proposed and the theoretical framework is outlined in this work. TSPE enables the classification between inhibitory and excitatory connections by using recorded action potentials. To compare this method learning about state of the art algorithms to estimate connectivity is necessary. After a research, promising algorithms are implemented and evaluated for further research topics, among others in the biomems lab of UAS Aschaffenburg. To evaluate these algorithms in silico networks are used, because of their known connectivity. This makes it possible to validate the correctness of our algorithm results. Therefore, a biophysically representative neuronal network simulation is needed first. Datasets were simulated in different ways and analysed in order to develop an evaluation framework. After a successful evaluation with in silico networks, in vitro experiments and their analyses complete this project.

==> content/1.tex <==
\chapter{Abschnitt}
Text\index{Abschnitt!Text} Text Text \EUR{83,50} Text Text Text Text Text\footnote{\cite[Vgl.][210]{Musteraufsatz}.} Text Text Text Text Text Text Text Text Text Text Text\footnote{\cite[Vgl. Heiner][215]{Musterbuch}.} Text Text Text Text \EUR{150,93} Text Text Text \euro Text Text Text. \footnote{\rcite{bmf021007}}

Text Text Text \EUR{83,50} Text Text Text Text Text\footnote{\cite[Vgl.][210]{Musteraufsatz}.} Text Text Text Text Text Text Text Text Text Text Text\footnote{\cite[Vgl. Heiner][215]{Musterbuch}.} Text Text Text Text \EUR{150,93} Text Text Text. \footnote{\rcite{bfh090319}}

Text Text Text \EUR{83,50} Text Text Text Text Text\footnote{\cite[Vgl.][210]{Musteraufsatz}.} Text Text Text Text Text Text Text Text Text Text Text\footnote{\cite[Vgl. Heiner][215]{Musterbuch}.} Text Text Text Text \EUR{150,93} Text Text Text. \footnote{\rcite{bfh060314}}
\section{Unterabschnitt}
Text Text Text \EUR{83,50} Text Text Text Text Text\footnote{\cite[Vgl.][210]{Musteraufsatz}.} Text Text Text Text Text Text Text Text Text Text Text\footnote{\cite[Vgl. Heiner][215]{Musterbuch}.} Text Text Text Text \EUR{150,93} Text Text Text. \footnote{\rcite{fg030925}}
\begin{itemize}
\item Punkt
\item Punkt
\item Punkt\footnote{\cite[Brox][212]{Musterbuch2}.}
\end{itemize}
\subsection{Unterabschnitt}
\begin{enumerate}
	\item $E_{ges}=m_{D}*c^{2}=\frac{m_{0}}{\sqrt{1-\frac{v^{2}}{c^{2}}}}$\index{Unterabschnitt!Formel}
\item $t-t_{0}=\sqrt{\frac{l}{g}}\int_{0}^{\varphi}{\frac{d\psi}{\sqrt{1-k^{2}\sin^{2} {\psi}}}} = \sqrt{\frac{l}{g}} F(k,\varphi)$
\item $u(x,t)= 8 \frac{k_{1}^{2}e^{\alpha_{1}} + k_{2}^{2}e^{\alpha_{2}} + (k_{1}-k_{2})^{2}e^{(\alpha_{1}+ \alpha_{2})} \left[2 + \frac{1}{(k_{1} + k_{2})^{2}} ( k_{1}^{2}e^{\alpha_{1}} + k_{2}^{2}e^{\alpha_{2}}) \right]}{\left[1+e^{\alpha_{1}} + e^{\alpha_{2}} + \left(\frac{k_{1} - k_{2}}{k_{1}+k_{2}} \right)^{2} e^{\alpha_{1}+ \alpha_{2}} \right]^{2}}$\footnote{\cite[Vgl.][23]{Musteraufsatz}.}
\end{enumerate}
\clearpage
\subsubsection{Unterabschnitt}
\begin{table}[ht]
\centering
\begin{tabular}{|c |c |}
\hline
\textbf{Erste Spalte} & \textbf{Zweite Spalte}\\% [0.5ex]
\hline\hline
Text & Text\\
\hline
Text & Text\\
\hline
Text & Text\\
\hline
Text & Text\\
\hline
Text & Text\\% [1ex]
\hline
\end{tabular}
\label{table:nonlin}
\caption[dieser Text steht im Tabellenverzeichnis]{Dieser Text steht bei der Tabelle} 
\end{table}
\paragraph{Unterabschnitt}
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=6cm]{./pic/logo-aschaffenburg.jpg}
\end{center}
\caption[dieser Text steht im Abbildungsverzeichnis]{Dieser Text steht beim Bild} 
\end{figure}
\subparagraph{Unterabschnitt}

\quote{\glqq \dots im vorliegenden Fall scheint die Beschwerdeführerin\index{Beschwerdeführering} in engem wirtschaftlichem Zusammenhang mit der GmbH und ihren Teilhabern zu stehen. Wenn dies der Fall ist, so dürfte unter Umständen ein einheitlicher Gewerbebetrieb in Frage kommen, zu dem einerseits das von der OHG verwaltete Fabrikgrundstück, ferner auch die GmbH-Anteile, soweit sie im Besitz der Gesellschaft der OHG sind, gehören würden.\grqq}

\chapter{Abschnitt}

\begin{figure}[ht]
\fbox{
\begin{minipage}[c]{0.95\textwidth}

\begin{minipage}[c]{0.94\textwidth}
\subparagraph*{\underline{Bruttoausweis:}}
\centering
\begin{tabular}{lr|lr}
\multicolumn{2}{l}{Aktiva} &
\multicolumn{2}{r}{Passiva} \\
\hline           
Ausstehende Einlage & 400           &   A. Eigenkapital                &        \\
Davon eingefordert  & 40~~~~     &   ~~~I. Gezeichnetes Kapital & 900    \\
\end{tabular}

~

~

\end{minipage}


\begin{minipage}[c]{0.94\textwidth}
\subparagraph*{\underline{Nettoausweis:}}
\centering
\begin{tabular}{lr|lr}
\multicolumn{2}{l}{Aktiva} &
\multicolumn{2}{r}{Passiva} \\
\hline           
B. Umlaufvermögen             &         &   A. Eigenkapital              &                    \\
~~~II. Forderungen            &         &   ~~~I. Gez. Kapital           & ~~~900             \\
~~~~~~~eingeford. Einlage     & 40~~~~  &   ~~~~~~nicht eingeford.       &                    \\
                              &         &   ~~~~~~Kapital                & ./.360             \\
                              &         &                                & --------           \\
                              &         &   ~~~~~~Eingeford. Kapital     & ~~~540             \\
\end{tabular}
\end{minipage}

\end{minipage}
}
\caption[Ausweis der ausstehenden Einlage]{Ausweis der ausstehenden Einlage}
\label{fig:gez_kap}
\end{figure}

